Improving Natural Language Inference with a Pretrained Parser

We introduce a novel approach to incorporate syntax into natural language inference (NLI) models. Our method uses contextual token-level vector representations from a pretrained dependency parser. Like other contextual embedders, our method is broadly applicable to any neural model. We experiment with four strong NLI models (decomposable attention model, ESIM, BERT, and MT-DNN), and show consistent benefit to accuracy across three NLI benchmarks.

==> figures/bert-scitail-confusion-mats.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/bert-scitail-cm.pdf}
    \includegraphics[width=0.45\linewidth]{figures/bert-lf-scitail-cm.pdf}
    \caption{Confusion matrices for BERT (left) and BERT\texttt{+LF} (right) on SciTail.}
\label{fig:bert-scitail-confusion-mats}
\end{figure*}

==> figures/da-scitail-confusion-mats.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/da-scitail-cm.pdf}
    \includegraphics[width=0.45\linewidth]{figures/da-sa-scitail-cm.pdf}
    \caption{Confusion matrices for DA (left) and DA\texttt{+SA} (right) on SciTail.}
\label{fig:da-scitail-confusion-mats}
\end{figure*}

==> figures/da-snli-confusion-mats.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/da-snli-cm.pdf}
    \includegraphics[width=0.45\linewidth]{figures/da-lf-snli-cm.pdf}
    \caption{Confusion matrices for DA (left) and DA\texttt{+LF} (right) on SNLI.}
\label{fig:da-snli-confusion-mats}
\end{figure*}

==> figures/esim-scitail-confusion-mats.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/esim-scitail-cm.pdf}
    \includegraphics[width=0.45\linewidth]{figures/esim-sa-scitail-cm.pdf}
    \caption{Confusion matrices for ESIM (left) and ESIM\texttt{+SA} (right) on SciTail.}
\label{fig:esim-scitail-confusion-mats}
\end{figure*}

==> figures/hans-tab-multinli.tex <==
\begin{table*}[tb]
\centering
\begin{tabular}{lcccccc}
\toprule
      & \multicolumn{3}{c}{Correct: \emph{Entailment}} & \multicolumn{3}{c}{Correct: \emph{Non-entailment}} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}
Model & Lexical & Subseq. & Const. & Lexical & Subseq. & Const. \\
\midrule
DA \citep{mccoy2019right}   & 0.99 & \textbf{1.00} & 0.97 & 0.01 & \textbf{0.02} & 0.03 \\
DA (ours) & \textbf{1.00} & \textbf{1.00} & \textbf{0.99} & 0.00 & 0.00 & 0.03 \\
DA + S & \textbf{1.00} & \textbf{1.00} & 0.98 & 0.00 & 0.00 & 0.03 \\
DA + SA & 0.98 & \textbf{1.00} & 0.97& \textbf{0.04} & \textbf{0.02} & \textbf{0.05} \\
\midrule
ESIM (ours) & 0.97          & 0.99 & \textbf{0.98} & \textbf{0.02} & \textbf{0.04} & \textbf{0.01} \\
ESIM + S    & \textbf{0.98} & 0.99          & \textbf{0.98} & 0.01 & \textbf{0.04} & \textbf{0.01} \\
ESIM + SA   & \textbf{0.98} & \textbf{1.00} & \textbf{0.98} & \textbf{0.02} & 0.03  & \textbf{0.01}-  \\
\midrule
BERT \citep{mccoy2019right} & 0.95    & 0.99    & 0.98   & 0.16    & 0.04    & \textbf{0.16}   \\
BERT (ours) & 0.97 & \textbf{1.00} & 0.99 & 0.65 & 0.11 & 0.10 \\
BERT + S & \textbf{0.98} & \textbf{1.00} & \textbf{1.00} & \textbf{0.66} & \textbf{0.13} & 0.12 \\
\midrule
MT-DNN (ours) & 0.95 & 1.00 & \textbf{0.99} & \textbf{0.83} & \textbf{0.14} & \textbf{0.21} \\
MT-DNN + S & \textbf{0.96} & \textbf{1.00} & \textbf{0.99} & 0.80 & 0.11 & 0.14 \\
\bottomrule
\end{tabular}
\caption{HANS stuff}
\label{table:hans-multinli}
\end{table*}


==> figures/mtdnn-scitail-confusion-mats.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/mtdnn-scitail-cm.pdf}
    \includegraphics[width=0.45\linewidth]{figures/mtdnn-lf-scitail-cm.pdf}
    \caption{Confusion matrices for MT-DNN (left) and MT-DNN\texttt{+LF} (right) on SciTail.}
\label{fig:mtdnn-scitail-confusion-mats}
\end{figure*}
